Designing and Evaluating Speech Emotion Recognition Systems: A reality check case study with IEMOCAP

There is an imminent need for guidelines and standard test sets to allow direct and fair comparisons of speech emotion recognition (SER). While resources, such as the Interactive Emotional Dyadic Motion Capture (IEMOCAP) database, have emerged as widely-adopted reference corpora for researchers to develop and test models for SER, published work reveals a wide range of assumptions and variety in its use that challenge reproducibility and generalization. Based on a critical review of the latest advances in SER using IEMOCAP as the use case, our work aims at two contributions: First, using an analysis of the recent literature, including assumptions made and metrics used therein, we provide a set of SER evaluation guidelines. Second, using recent publications with open-sourced implementations, we focus on reproducibility assessment in SER.

==> tables/table1.tex <==
\begin{table*}[!ht]
    \footnotesize
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
       & & & & & \multicolumn{2}{c}{Performance} & \\
       & & & & & & & & \\ 
       \# & Publication & Venue & Code & Acoustic Feats & UA (\%) & WA (\%) & cross-val & Comments on Eval.\\
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8} \cmidrule(lr){9-9} 
      1 & Feng et al.~\cite{feng20_interspeech}& Interspeech20 & \href{https://github.com/Kyoto-University-Speech-and-Audio/feng-asr-ser}{Yes} & MFCCs & 76.4 & 75.5 & 5-fold & -\\
      2 & Zhu and Li~\cite{zhu2022speech}      & ICASSP22      & \href{https://github.com/lixiangucas01/GLAM}{Yes} & MFCCs & 73.90 & 73.70 & 5-fold  & Excited as Happy\\
      3 & Xu et al.~\cite{xu2020improve}       & CCWC20        & \href{https://github.com/lessonxmk/head_fusion}{Yes} & Spectrograms  & 67.94 & 67.28 & 5-fold  & Excited as Happy \\
    %\cmidrule{1-8}
      4 & Gat et al.~\cite{gat2022speaker}     & ICASSP22   & No & HuBERT & - & 81.0 & 5-fold & -\\
      5 & \multirow{2}{*}{Wang et al.~\cite{wang2021fine}}  &  \multirow{2}{*}{Preprint} & \multirow{2}{*}{\href{https://github.com/speechbrain/speechbrain/tree/develop/recipes}{Yes}}        & HuBERT & 79.58 & -  & \multirow{2}{*}{5-fold} & - \\
      6 &                                                   &  &                             & w2v2   & 77.47 & -  &  & -\\ 
      7 & Peng et al.~\cite{peng2021efficient} & ICASSP21 & No & MFCCs & 79.1 & 78.0 & 10-fold & -\\ 
    \cmidrule{1-9}
      8 & Xu et al.~\cite{xu2021speech}        & ICASSP21           & \href{https://github.com/lessonxmk/Optimized_attention_for_SER}{Yes} & Spectrograms  & 77.54 & 79.34 & 5-fold  & Improv. only, Excited as Happy\\
      9 & Xu et al.~\cite{xu2020improve}       & CCWC20             & \href{https://github.com/lessonxmk/head_fusion}{Yes}                 & Spectrograms  & 76.36 & 76.18 & 5-fold  & Improv. only, Excited as Happy \\
      10 & Xu et al.~\cite{xu2020improve}       & CCWC20             & \href{https://github.com/lessonxmk/head_fusion}{Yes}                 & Spectrograms  & 63.92 & 65.90 & 5-fold  & Scripted. only, Excited as Happy \\
      11 & Zhu and Li~\cite{zhu2022speech}      & ICASSP22          & \href{https://github.com/lixiangucas01/GLAM}{Yes}                    & MFCCs & 79.25 & 81.18 & 5-fold  & Improv. only, Excited as Happy \\
      12 & Zhu and Li~\cite{zhu2022speech}      & ICASSP22          & \href{https://github.com/lixiangucas01/GLAM}{Yes}                    & MFCCs & 70.39 & 71.44 & 5-fold  & Scripted only, Excited as Happy \\
      13 & Liu and Wang~\cite{liu21n_interspeech} & Interspeech21   & No                                                                   & MFCCs & 78.30 & 79.52 & 5-fold  & Imrpov. only \\
      14 & Moine et al.~\cite{moine21_interspeech} & Interspeech21  & No                                                                   & Spectrograms  & 77.22 & -     & 5-fold  & Imrpov. only\\
    \bottomrule
    \end{tabular}
    
    \caption{Comparison of methods that perform Speaker Dependent (SD) evaluation. Rows 8-12 perform random 5-fold cross val. only on the improvised data. Still, the comparison isn't fair because they randomly create the test set.}
    \label{table1}
\end{table*}

==> tables/table1_v2.tex <==
\begin{table*}[!ht]
    \footnotesize
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
       & & & & & \multicolumn{2}{c}{Performance} & \\
       & & & & & & & & \\ 
       \# & Publication & Venue & Code & Acoustic Feats & UA (\%) & WA (\%) & cross-val & Comments on Eval.\\
      \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8} \cmidrule(lr){9-9} 
      1 & Feng et al.~\cite{feng20_interspeech}& Interspeech20 & \href{https://github.com/Kyoto-University-Speech-and-Audio/feng-asr-ser}{Yes} & MFCCs & 76.4 & 75.5 & 5-fold & -\\
      2 & Zhu and Li~\cite{zhu2022speech}      & ICASSP22      & \href{https://github.com/lixiangucas01/GLAM}{Yes} & MFCCs & 73.90 & 73.70 & 5-fold  & Excited as Happy\\
      3 & Xu et al.~\cite{xu2020improve}       & CCWC20        & \href{https://github.com/lessonxmk/head_fusion}{Yes} & Spectrograms  & 67.94 & 67.28 & 5-fold  & Excited as Happy \\
    %\cmidrule{1-8}
      4 & Gat et al.~\cite{gat2022speaker}     & ICASSP22   & No & HuBERT & - & 81.0 & 5-fold & -\\
      5 & \multirow{2}{*}{Wang et al.~\cite{wang2021fine}}  &  \multirow{2}{*}{Preprint} & \multirow{2}{*}{\href{https://github.com/speechbrain/speechbrain/tree/develop/recipes}{Yes}}        & HuBERT & 79.58 & -  & \multirow{2}{*}{5-fold} & - \\
      6 &                                                   &  &                             & w2v2   & 77.47 & -  &  & -\\ 
      7 & Peng et al.~\cite{peng2021efficient} & ICASSP21 & No & MFCCs & 79.1 & 78.0 & 10-fold & -\\ 
    \cmidrule{1-9}
      8 & Xu et al.~\cite{xu2021speech}        & ICASSP21           & \href{https://github.com/lessonxmk/Optimized_attention_for_SER}{Yes} & Spectrograms  & 77.54 & 79.34 & 5-fold  & Improv. only, Exc. as Hap.\\
      9 & Xu et al.~\cite{xu2020improve}       & CCWC20             & \href{https://github.com/lessonxmk/head_fusion}{Yes}                 & Spectrograms  & 76.36 (63.92) & 76.18 (65.90) & 5-fold  & Improv. (Scripted) only, Exc. as Hap. \\
      10 & Zhu and Li~\cite{zhu2022speech}      & ICASSP22          & \href{https://github.com/lixiangucas01/GLAM}{Yes}                    & MFCCs & 79.25 (70.39) & 81.18 (71.44) & 5-fold  & Improv. (Scripted) only, Exc. as Hap. \\
      11 & Liu and Wang~\cite{liu21n_interspeech} & Interspeech21   & No                                                                   & MFCCs & 78.30 & 79.52 & 5-fold  & Imrpov. only \\
      12 & Moine et al.~\cite{moine21_interspeech} & Interspeech21  & No                                                                   & Spectrograms  & 77.22 & -     & 5-fold  & Imrpov. only\\
    \bottomrule
    \end{tabular}
    
    \caption{Comparison of methods that perform Speaker Dependent (SD) evaluation. Rows 8-12 perform random 5-fold cross val. only on the improvised data. Still, the comparison isn't fair because they randomly create the test set.}
    \label{table1}
\end{table*}

==> tables/table2.tex <==
\begin{table*}[!ht]
    \footnotesize
    \centering
    \begin{tabular}{cccccccc}
    \toprule
       & & & & & \multicolumn{2}{c}{Performance} & \\
       & & & & & & & \\ 
       \# & Publication & Venue & Code & Acoustic Feats & UA (\%) & WA (\%) & cross-val\\
   \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3}  \cmidrule(lr){4-4} \cmidrule(lr){5-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-8} 
      %1 & Pepino et al.~\cite{pepino21_interspeech} & Interspeech21   & \href{https://github.com/habla-liaa/ser-with-w2v2}{Yes} & w2v2 & 67.2 & - & 5-fold \\
      2 & Yang et al.~\cite{yang21c_interspeech}    & Interspeech21   & \href{https://github.com/s3prl/s3prl}{Yes} & HuBERT & 67.62 & -    &  5-fold \\
      3 & Gat et al.~\cite{gat2022speaker}          & ICASSP22        & No & HuBERT & -     & 74.2 & 5-fold \\
      4 & Santoso et al.~\cite{santoso21_interspeech} & Interspeech21 & No & MFCC+CQT+F0 & 75.9 & 76.1   & 5-fold \\
      5 & Li et al.~\cite{li19n_interspeech}        & Interspeech19   & \href{https://github.com/KrishnaDN/speech-emotion-recognition-using-self-attention}{No} & Spectrograms & 82.8 & 81.6 & 5-fold \\
    %\cmidrule{1-8}
      6 & \multirow{2}{*}{Zou et al.~\cite{zou2022speech}}     &  \multirow{2}{*}{ICASSP22} &  \multirow{2}{*}{\href{https://github.com/vincent-zhq/ca-mser}{Yes}} &  \multirow{2}{*}{MFCCs,Spec,w2v2} & 71.05 & 69.80 & 5-fold \\ 
      7 & & & & & 72.70 & 71.64 & 10-fold \\ 
      8 & \multirow{2}{*}{Wang et al.~\cite{wang2021fine}}  &  \multirow{2}{*}{Preprint} & \multirow{2}{*}{\href{https://github.com/speechbrain/speechbrain/tree/develop/recipes}{Yes}}        & HuBERT & 73.01 & -  & \multirow{2}{*}{10-fold}  \\
      9 &                                                   &  &                             & w2v2   & 70.99 & -  &  \\ 
      10 & Aftab et al.~\cite{aftab22lightsrnet} & ICASSP22 & \href{https://github.com/AryaAftab/LIGHT-SERNET}{Yes} & MFCCs & 70.76 & 70.23 & 10-fold \\
      11 & Feng et al.~\cite{feng20_interspeech}& Interspeech20 & \href{https://github.com/Kyoto-University-Speech-and-Audio/feng-asr-ser}{Yes} & MFCCs & 69.67 & 68.63 & 10-fold \\
      12 & Cai et al.~\cite{cai21b_interspeech} & Interspeech21 & \href{https://github.com/TideDancer/interspeech21_emotion}{Yes} & w2v2 & - & 78.15 & 10-fold \\
      13 & Shor et al.~\cite{shor2022universal}          & ICASSP22      & No                                                  & CAP & - & 79.2  & Session 05  \\
      14 & Shor and Venugopalan~\cite{shor2022trillsson} & Interspeech22 & \href{https://tfhub.dev/s?q=trillsson}{Yes} \hyperref[trill]{\dag}  & \textsc{TRILLsson} & - &  73.2 & Session 05 \\
    \bottomrule
    \end{tabular}
    
    \caption{Comparison of methods that perform Speaker Independent (SI) evaluation. The works of rows 11,12 use Session05 (i.e. speakers '05M' and '05F') as test set. \label{trill}(\dag): They provide the weights for their pre-trained models. }
    \label{table2}
\end{table*}
